Off-Path Attacking the Web

We show how an off-path (spoofing-only) attacker can perform cross-site scripting (XSS), cross-site request forgery (CSRF) and site spoofing/defacement attacks, without requiring vulnerabilities in either web-browser or server and circumventing known defenses. Attacker can also launch devastating denial of service (DoS) attacks, even when the connection between the client and the server is secured with SSL/TLS. The attacks are practical and require a puppet (malicious script in browser sandbox) running on a the victim client machine, and attacker capable of IP-spoofing on the Internet. Our attacks use a technique allowing an off-path attacker to learn the sequence numbers of both client and server in a TCP connection. The technique exploits the fact that many computers, in particular those running Windows, use a global IP-ID counter, which provides a side channel allowing efficient exposure of the connection sequence numbers. We present results of experiments evaluating the learning technique and the attacks that exploit it. Finally, we present practical defenses that can be deployed at the firewall level; no changes to existing TCP/IP stacks are required.

==> BehindNAT.tex <==
\section{Exposing the Client Port Behind a Randomizing NAT} \label{appendix:clientport}

In this section we describe a probing technique that allows an off-path (blind) adversary, \mal, to identify a connection between a client \wini\ and a server \lin\ when \wini\ is using a globally incrementing IP identifier (IP-ID), but is behind a NAT or a firewall that randomizes the client port. The attacker not only identifies the existence of the connection, but also learns the client port.

The following subsection defines a {\em port test} that uses the leakage in the IP-ID field to detect whether \wini\ is communicating with \lin\ through a tested port. In order to detect whether a connection between them exists, this test is applied on ports that \wini\ is `likely' to use as a source port for a connection with \lin. There are $2^{16}$ possible TCP ports; we could test all of them. However, in Windows, ports are also allocated sequentially; therefore, \mal\ can assume that if \wini\ is communicating with \lin, then the source port \wini\ is using for \lin\ is `close' to the port that \wini\ is using for the connection with \mal. This observation significantly improves this attack vector, as we show in the experiments below.

Once we decided upon the set of ports to be tested, we perform the test for all of them. We keep a `score' for each possible port, and increment a specific port's score by $1$ point for every test that seems to indicate that there is a connection through that port. As we show in experimental runs in this section, and analyze later, errors are likely to occur (e.g., if the victim sends an independent packet while the test takes place). Thus, we conduct $r > 1$ rounds of the attack, where each port is tested. Finally, we decide that there is a connection if there is a port with a score higher than a threshold, \textit{TH}.

\ignore{ Subsection \ref{Privacy:ID:Analysis} provides a probabilistic modeling and analysis for ID based probing techniques and compares between the two variants. Finally, }

\subsection{The Client Port Test} \label{Privacy:ID:FW}

According to the TCP specification \cite{rfc793} (Section 3.9, bottom of page 69), the first check that a receiver conducts on an incoming packet (in case it belongs to an established connection) validates that the sequence number is within the flow control window. If this check finds the packet invalid, then the recipient discards it and sends a duplicate Ack feedback to the source. A stateful firewall or NAT device connecting \wini\ to the network keeps track of existing connections and processes all incoming packets before they reach \wini. We use the following observation: incoming packets that do not belong to an established connection will be discarded before reaching \wini\ (by firewall/NAT), whereas packets that belong to an existing connection, but specify arbitrary (probably invalid) sequence numbers will reach \wini\ who replies with a duplicate Ack.

The port test for the case of NAT/FW deploying client is illustrated in Figure \ref{fig:PortTest}, and is according to the general query-probe-query pattern. The probe specifies \lin's address and port as source (i.e., probe is spoofed) and \wini's address as destination, \mal\ specifies a different destination port in each test. Notice that since the probe packet appears to be from \lin\ (in case it specifies a valid 4-tuple), it is difficult to block the probe in firewalls without blocking the legitimate connection that \wini\ has with \lin.

\begin{figure}
	\vspace{-10pt}
	\centering
		\includegraphics[width=0.41\textwidth]{PortTest.pdf}
	\caption{Two iterations of port test. In the first iteration the firewall/NAT blocks the probe packet (i.e., no connection through the tested port). In the second iteration the probe specifies existing connection parameters (IP addresses and ports) and therefore reaches \wini\ who processes the probe and sends a duplicate Ack to \lin.\ignore{; this delays processing of the corresponding post probe query.}}
	\label{fig:PortTest}
	\vspace{-10pt}
\end{figure}

When \wini\ uses a global identifier, the difference in the IP-ID field in \wini's responses to \mal\ indicates whether \wini\ had sent a packet in response to the probe (duplicate Ack). If \mal\ identifies that \wini\ had sent a packet, then it is likely that \wini\ is communicating with \lin\ via the tested port. Repeating this test several times allows \mal\ to efficiently detect whether \wini\ is connected to \lin\ and reveal \wini's port in this case; see our empirical results below.

Some firewalls have an option to randomize the IP-ID; our tests would, of course, fail if the packets pass through such randomizing firewall. However, from our experience these are not common.

\subsection{Empirical Evaluation} \label{Privacy:ID:Results}

We first evaluated the attack in case that \wini\ is communicating with \lin. We compared between the score of the `connection port' (i.e., port that \wini\ uses for the connection) to that of the best appearing non-connection port (i.e., port with the highest score that is not the connection port) in each round \footnote{A round is a repetition of the attack, see discussion above.}; note that the highest scoring non-connection port may change between rounds. Figure \ref{fig:Privacy:ID:Scoreboard} illustrates our results in two environments for the in-campus and the off-campus attackers. The figure shows that using the global-ID as a side channel, an attacker can distinguish between connection to non connection ports.

\begin{figure}
	\centering
		\includegraphics[width=0.45\textwidth]{ID-Scoreboard.eps}
		\caption{Global-ID attack. Comparison of a connection port to that of the highest scoring non connection port as a function of round number. Each measurement is an average of $10$ runs, error-bars mark the standard deviation values.}
		\label{fig:Privacy:ID:Scoreboard}
		\vspace{-10pt}
\end{figure}

Figure \ref{fig:Privacy:ID:Scoreboard} shows that in both environments the score of the connection port was well above $50\%$ of the maximal score in each round. This motivates to continue testing only `high scoring' ports in advanced rounds. Namely, a port is tested in the next round only if its current score is above $50\%$ of the maximal possible score. 

We implemented an adversarial website that presents its clients a request to arbitrarily decide whether to connect (`surf') to a third-party website, \lin; our website attempted to detect the clients' choice. We used an automatic client, \wini, that chooses to connect to \lin\ with probability $\frac{1}{2}$ and implemented the port-test for the case that the \wini\ connects through a NAT or a firewall.

The choice of whether there is a connection between \wini\ and \lin\ is according to a threshold over the final score of the ports. Namely, if there exists a port with a score over this threshold, then we identify that there is a connection. Figure \ref{fig:Privacy:ID:Scoreboard} shows that a choice of $70\%$ of the maximal possible score as a threshold provides a good seperation between the connection port (in case it exists) and other ports. Figure \ref{fig:Privacy:ID:Internet} shows the success rate in detecting whether \wini\ communicates with \lin\ for different adversary locations as a function of the duration of the attack. Figure \ref{fig:Privacy:ID:Tests} compares the average amount of data that \mal\ sends (per victim) to reach different success rates and for different locations in the network. 

In Figure \ref{fig:Privacy:ID:Tests}, the measurements are the average of $50$ runs; error-bars mark the standard deviation values (for readability, not all measurements specify the error bars).

%For all three locations, the longer the measurement in the attack, the less additional tests that \mal\ is performs since there are less ports to re-check (i.e., ports that did not fall below the round-threshold).

 %The figure compares between Internet and LAN environments as a function of the number of rounds.


\begin{figure}[ht]
\centering
		\includegraphics[width=0.45\textwidth]{IDInternet.eps}
		\caption{Global-ID attack, Internet attacker (delay of 200ms and jitter).}
		\label{fig:Privacy:ID:Internet}
		
\end{figure}

\begin{figure}
\centering
		\includegraphics[width=0.45\textwidth]{IDTests.eps}
		\caption{Amount of data \mal\ sends as a function of his success rate.}
		\label{fig:Privacy:ID:Tests}
\end{figure}

==> DoS.tex <==
\section{Brief Discussion on Denial of Service} \label{Injection:DoS}

Can deny even SSL traffic, MTA servers.......
Given connection params no need to \wini, no need for sequence numbers.


==> DosAttacks.tex <==
\section{DoS} \label{DoS}
TBD:

\begin{enumerate}
	\item How to form a connection with Lin and get the port
	\item Launching Ack Storm
	\item Launching Opt Ack
\end{enumerate}





==> IDErrors.tex <==
\section{Sequence Exposure - Error Rate Probability} \label{errorrate}
Assume that \wini\ outputs packets according to the Poisson distribution, denote by $\lambda$ the expected number of `independent' packets that \wini\ sends per second (i.e., packets that do not relate to the sequence test). The three packets in the test arrive and handled by \wini\ very closely to each other, in a short time interval; denote its length by $\tau$. The probability that \wini\ sends at least one independent packet of the test during the sensitive time interval is $1 - e^{-\lambda\tau}$. 


Consider an example where $\lambda = 32, \tau = 0.1$ ms, then the probability that \wini\ sends a packet during the test is $p = 0.25\%$. \mal\ conducts $\frac{2^{32}}{\textit{wnd-size}}$, but only in one of them she should indicate \wini\ did not send a packet. When \mal\ conducts a binary search for the exact value of the sequence number (see end of Section \ref{Injection:SeqExposure:learning}), he conducts $\log_2(\textit{wnd-size})$; if $\textit{wnd-size} = 2^{16}$, then there are 16 iterations; on average, 8 iterations should indicate that no packet was sent.
Similarly, there are $32$ client-sequence tests during the binary search for the client sequence number, on average 16 tests should indicate that the probe did not cause \wini\ to send any packet. \mal\ errors if \wini\ sends an independent packet during these tests. The probability that this event occurs is $1 - (1 - p)^{1 + 8 + 16} \approx 0.06$.

==> Model.tex <==
\section{Model and Technique} \label{Injection:Model}

Let \wini\ and \lin\ be communicating TCP client and server (respectively). We assume that \wini\ is a Windows client and leverage side channels that exist in Windows TCP/IP implementation to perform our attacks. The vast deployment of Windows on client machines (more than $80\%$ according to browser user-agent based surveys, see \cite{Wikimedia}) makes our assumption and attacks very practical. 

The adversary, we name \mal, is able to send {\em spoofed packets}; i.e., able to send packets containing incorrect sender IP address. The IETF recommends that Internet Service Providers (ISPs) will block packets from their customers that specify source IP address not assigned to the sender, i.e., {\em ingress filtering} \cite{rfc3013,rfc2827,rfc3704}. Indeed, \cite{SpooferProject} found that most surveyed clients were unable to send spoofed packets. However, there are still many ISPs that do not perform ingress filtering. In particular, \cite{pang2004cib,beverly2005spi} found that IP spoofing and lack of ingress filtering are still quite common.

Cyber warfare - ingress filtering relies on cooperation, while BGP hijacks performed by some governments seem to be detected it is much harder to detect IP spoofing, and governments can perform it simply since they control the ISPs.


\mal\ is an off-path attacker who we assume cannot eavesdrop on either \wini\ or \lin. We make a much weaker assumption: \mal\ can communicate with \wini, e.g., since \wini's browser will send a request to \mal. The typical case that we consider is that \mal\ persuades the victim, \wini, to connect to his website. \mal\ uses this (legitimate) connection, to probe a connection that \wini\ has with another site, \lin, see Figure \ref{fig:AttackSite}. We present the probing technique in the following sections.

\ignore{
Namely, \mal's queries (see Figure \ref{fig:3PhaseTest}) are data packets sent on the connection between \mal\ and \wini, and the responses are \wini's TCP acknowledgments.}

In our initial discussions presenting the sequence numbers exposure attack we assume that \mal\ has the TCP four tuple describing a connection between \wini\ and \lin. Namely, \mal\ knows their IP addresses and ports. Later in Section \ref{DoS} we show how \mal\ can obtain these parameters by forming a {\em new} connection between \wini\ and \lin\ (when \wini\ enters \mal's website).

\begin{wrapfigure}{r}{0.5\textwidth}
\centering
		\includegraphics[width=0.47\textwidth]{Mal.pdf}
		\caption{\mal\ uses the connection he has with \wini\ to probe the connection that \wini\ has with \lin.}
		\label{fig:AttackSite}
\end{wrapfigure}


==> NoFW.tex <==
\section{Obtaining Address and Port of a Non-Protected Client} \label{Injection:NoFW}

If \wini\ is not protected by a firewall, then the 3-packet port test that we provided in Section \ref{Injection:Client} will not be helpful, since in any case \wini\ will output a packet: either a duplicate acknowledgment, in case that the middle packet specifies correct parameters; or RST, in the other case.

We next define a different 3-packet test that uses the server, \lin, to indirectly probe \wini, this technique is a variant of the idle port scan \cite{IdleScan}.
Denote by $\delta^l_m, \delta^w_l, \delta^w_m$ average network delays from \mal\ to \lin, from \lin\ to \wini\ and from \mal\ to \wini\ respectively. Let $\epsilon$ be some small time constant.

In the modified version, \mal\ sends at time $0$ a SYN packet to \lin; that specifies \wini\ as source and a port. In case that the SYN specifies parameters (IP addresses, and Ports) of a valid connection, \lin\ believes that \wini\ is a new client and sends a SYN, ACK packet in response to continue the three way handshake. This will cause \wini\ to send back a RST packet (since he did not send the corresponding SYN to \lin). In case that the SYN belongs to an established connection between \lin\ and \wini, \lin\ is likely to send a duplicate ACK since the sequence number is likely to be invalid (otherwise, if the sequence number is valid, \lin\ tears down the connection), the duplicate ACK will not cause \wini\ to send any packet in response since it does not contain any data (see related discussion in Section \ref{Injection:SeqAck:Seq}).

At time $\delta^l_m + \delta^w_l - \delta^w_m - \epsilon$ \mal\ sends a query packet to \wini, and sends an additional 
query at time $\delta^l_m + \delta^w_l - \delta^w_m + \epsilon$, if between the queries \wini\ receives \lin\ response to \mal's SYN packet, then he will be able to detect whether the specified port is correct.

==> OnSequences.tex <==
\section{The Challenge in (Blind) TCP Injection}

For an off-path adversary as \mal, detecting a valid sequence number is challenging (but this was not always the case, e.g., see \cite{zalewski2005silence}). TCP implementations today use a pseudo random function to choose an initial sequence number when the connection is established \cite{rfc1948}.

%check this statement below
According to the TCP specification \cite{rfc793}, a valid sequence number, as well as knowledge of a connection's IP addresses and ports, are enough to inject traffic (in one direction). Indeed this allows injection of traffic to Linux and various Windows (e.g., XP SP0) based machines. However more recent (and more common) versions of Windows (XP SP3, Vista, Win7) also require an incoming TCP packet to specify a valid 32-bit acknowledgment number. The acknowledgment is valid if it is for data that the recipient had sent, but were not acknowledged earlier; or in case that all data was acknowledged, the acknowledgment specifies the sequence number for the next packet that the receiver will send. 

To cope with this challenge we use a side channel given in the IP identifier field that \wini\ specifies in packets he sends. The IP identifier is important for reassembly of IP packets from their fragments, where the receiver must uniquely identify the set of fragments belonging to each packet. The IPv4 standard \cite{rfc791} does not specify how to choose the identifier, but many implementations use an incrementing identifier.

A globally-incrementing identifier is not really hidden from \mal, who can usually learn its value simply by receiving some packet from the victim. This is often possible as a response to a packet that \mal\ sends, e.g., SYN to public web server, SYN-ACK or RST to a closed client port, echo requests, etc. We refer to such packets as {\em queries} and to the corresponding packets that the victim sends as {\em responses}. Another common scenario where \mal\ is able to learn the global identifier, is when he persuades the victim to run a low privileged script, e.g., in a browser's sandbox when entering \mal's website.

The global identifier is operating system dependent; however it often exists. In particular, a globally incrementing IP identifier is used by Windows which is rather common, especially for client machines where its market share is more than $80\%$ according to Browser user-agent based survays, see \cite{Wikimedia}. Therefore, it is likely that \mal\ will be able to sample the current value of IP identifier of at least one peer in a connection. 

The global IP identifier allows \mal\ to probe for the number of packets that \wini\ sends. We use this observation in the sequence exposure attack described in the following section.

\subsection{Query-probe-query attack pattern} 
%In contrast, our results allow a spoofing-only attacker to expose TCP's sequence numbers as well as the client port, even when the initial sequence number and client port are selected randomly. Furthermore, we have successfully validated our results experimentally, see within. 
Our attacks can be viewed as instances of an {\em attack pattern} which we call {\em Query-Probe-Query}, illustrated in Figure \ref{QPQ:pattern:fig}; this is a generalization of the well-known {\em idle stealth scan} attack \cite{zalewski2005silence,Klein07:OpenBSD,nmap:book}, and of the measurement method used in \cite{conf/imc/Bellovin02}. 

Idle scan uses a client running Windows (or any system using globally-incrementing IP-ID) to test if some server has an open port, using three packets (or three phases). First, the attacker sends some {\em probe packet} to the client, to receive a response containing current IP-ID $i$. Second, the attacker sends a SYN packet to the server, using source IP address of client; if the port is open, client receives SYN-ACK and responds with RST, and if closed, client will receive RST and not send any response. Finally, attacker again sends probe packet to client, and receives current IP-ID $j$. If $j=i+1$, attacker concludes that no packet was sent (since server port was closed). 

In the {\em Query-Probe-Query attack pattern}, the first query measures some `pre-probe state'; the probe may cause some change on the state, where the change depends on the property measured, e.g., whether a specific port is open; and the final query  measures the `post-probe state'. This  attack pattern can be applied with different queries and probes,  to measure different values; see Figure \ref{fig:3PhaseTest}. 

In our implementations, each probe is a packet (or few packets) sent to the victim (usually Windows) machine \wini. The probes test for some event $e$, such that if $e$ holds then \wini\ will send some packet(s), and otherwise \wini\ will not send a packet (or send less packets). We can use two different query mechanisms (side channels): measure the IP-ID counter, or measure time between receipt of the different probe packets. 

\begin{figure}[htb]
	\centering
		\includegraphics[width=0.48\textwidth]{3PhaseTest.pdf}
	\caption{Query-Probe-Query Attack Pattern.}
	\label{fig:3PhaseTest} \label{QPQ:pattern:fig}
\end{figure}

%Our attack consists of several steps. First, the adversary, Mal, identifies that some client in a particular network is communicating with a specific server $S$; this first phase uses a simple (iterative) DNS query. Second, Mal scans the clients in the network, and finds the client \wini\ that communicates with $S$;   he also identifies the client port in the connection. Once Mal has identified the TCP connection (i.e., the four tuple), he sends to \wini\ probe packets that identify the current sequence numbers of the connection (in our experiments, this phase takes few seconds to few minutes, depending on the network parameters, delays, bandwidth , window size etc.). When Mal also has the relevant sequence numbers, he is able to inject data to the connection in both directions.


==> Parameters.tex <==
\section{Challenges} \label{Injection:Parameters}

In TCP injection attacks, the adversary, \mal, wishes to send a packet to a victim \wini\ (\lin) such that the packet's data will appear as part of \lin's (\wini's) data stream and reach the recipient's application layer. In this section we list the parameters that \mal\ needs to specify in his packet in order to conduct a successful attack, and discuss the challenges in obtaining their values. Some parameters are more general, e.g., also relevant for injecting spoofed UDP packets, some are TCP specific; parameters of the latter type are often considered more difficult to predict or study. 
The following sections introduce techniques for \mal\ to efficiently study {\em all} required parameters, allowing the injection attack, some parameters are also of independent interest (e.g., for traffic analysis) as we will show in the following section. A general challenge that our techniques must deal with is deployed firewalls, we refer to this challenge in the following sections.

\subsection{IP Addresses and Ports} \label{Injection:Parameters:Connection}

There are four parameters that uniquely identify a TCP connection between \wini\ and \lin, i.e. IP addresses and ports for both \wini\ and \lin. Trivially, in order conduct any attack on a TCP connection, Mal must identify it. 
%These parameters are also required for UDP injections.

Typically, in a TCP connection, one peer is the server and one is the client. The server's address and port are usually advertised or well known, and we assume that \mal\ has preliminary knowledge of them. However, the corresponding client parameters are somewhat hidden; yet \mal\ is not completely oblivious to the client's IP address: clients on the same network usually have IP addresses with the same prefix due to CIDR allocation \cite{rfc1519}; this is even more conspicuous in the hierarchic structure of IPv6 addresses \cite{rfc4291}. Namely, in many cases \mal\ can identify a relatively small set of possible addresses for a particular client, e.g., according to physical location, ISP, or organization. Additionally, many networks are connected via a Network Address Port Translator (NAPT) device, in this case, all connections with that network specify the NAPT's IP address; once \mal\ identifies this address, he obtained the address parameter for the entire network.

The 16-bit client port is usually not arbitrary as well. As apposed to recent recommendations \cite{rfc6056}, many operating systems, e.g., Windows, allocate ports sequentially, often even starting from a constant value (1024). In this case, some ports are generally more likely than others. 

\ignore{
In Section \ref{Injection:Client} we provide an attack that would identify if any client in a network is communicating with a server $S$ in a particular domain. Furthermore, given a specific IP address of suspected client, e.g. \wini, the attack would identify whether that particular \wini\ is communicating with a server $S$, in this case, the attack would also yield the \wini's port. For this phase we we use a time-based side channel attack which is applicable regardless of the victim's operating system. %The latter phase requires that the client uses a global IP-identifier (e.g., a windows machine).

This attack allows \mal\ to detect the connection parameters of a specific client or clients within small to medium networks and conduct the injection attack. Furthermore, this attack is also of independent interest since the adversary identifies that a particular client and server are communicating. 

We use the observations on address and port allocation above to improve the expected running time of the attack. 
}

\ignore{
if \mal\ is able to somehow create a connection with the suspected client, then he will be able to infer on corresponding port that client is using in his connection with the server. However, we identify three good reasons not to use this method:
\begin{enumerate}
	\item in many cases \mal\ is not able to establish connections with potential clients of $S$ 
	(in particular, SYN packets are often blocked by client firewalls).
	\item this method will not provide proof that a particular client is or is not communicating with $S$, 
	\mal\ may be wrong about the client he suspects.
	\item \mal\ does not receive the exact port (although the set of possible ports may be small, and allow him to attack all possibilities).
\end{enumerate}
}

\subsection{Sequence Numbers} \label{Injection:Parameters:SeqAck}

The 32-bit TCP sequence number indicates `where' the packet's data fits within the TCP connection stream;
it allows the recipient to cope with packet reordering, and identify packet loss as well as duplicates and invalid packets:
the receiver keeps a congestion window $\textit{cwnd}$ for every connection, and discards a packet $p$ if its sequence number indicates that $p$'s data is completely outside the limits of $\textit{cwnd}$. Thus, in order to inject a packet into the connection, \mal\ must specify a valid sequence number; i.e., such that at least some of the data is within the receiver's $\textit{cwnd}$. 

For a blind adversary, detecting a valid sequence number is challenging (but this was not always the case, e.g., see \cite{zalewski2005silence}). TCP implementations today use a pseudo random function to choose an initial sequence number when the connection is established \cite{rfc1948}.

\ignore{
For a blind adversary, detecting a valid sequence number is challenging. 
The once predictable initial sequence number, allowed blind adversaries (e.g., \mal) to setup `ghost' connections, i.e., TCP connections form spoofed addresses, the attack was first noticed in the 1980s, but gained attention only in 1995 \cite{morris1,Tsutomu}. Therefore, TCP implementations today use a pseudo random function to choose an initial sequence number when the connection is established \cite{rfc1948}, thereby preventing blind adversaries from completing the 3-way handshake \cite{rfc793}.
}

%check this statement below
According to the TCP specification \cite{rfc793}, a valid sequence number, as well as knowledge of a connection's IP addresses and ports, are enough to inject traffic (in one direction). Indeed this allows injection of traffic to Linux and various Windows (e.g., XP SP0) based machines. However more recent (and more common) versions of Windows (XP SP3, Vista, Win7) also require an incoming TCP packet to specify a valid 32-bit acknowledgment number. The acknowledgment is valid if it is for data that the recipient had sent, but were not acknowledged earlier; or in case that all data was acknowledged, the acknowledgment specifies the sequence number for the next packet that the receiver will send. 

\ignore{
We present a TCP sequence number learning attack in Section \ref{Injection:SeqAck} that allows \mal\ to obtain the sequence numbers used by \lin\ and \wini\ to send data. Thereby, the attack also provides \mal\ with valid acknowledgment numbers for both peers, allowing \mal\ to inject data in either direction. The attack requires that the victim would use a global IP-identifier (e.g., a windows machine).
}
